Conditional expectation with regularization for missing data imputation

Missing data frequently occurs in datasets across various domains, such as medicine, sports, and finance. In many cases, to enable proper and reliable analyses of such data, the missing values are often imputed, and it is necessary that the method used has a low root mean square error (RMSE) between the imputed and the true values. In addition, for some critical applications, it is also often a requirement that the imputation method is scalable and the logic behind the imputation is explainable, which is especially difficult for complex methods that are, for example, based on deep learning. Based on these considerations, we propose a new algorithm named "conditional Distribution-based Imputation of Missing Values with Regularization" (DIMV). DIMV operates by determining the conditional distribution of a feature that has missing entries, using the information from the fully observed features as a basis. As will be illustrated via experiments in the paper, DIMV (i) gives a low RMSE for the imputed values compared to state-of-the-art methods; (ii) fast and scalable; (iii) is explainable as coefficients in a regression model, allowing reliable and trustable analysis, makes it a suitable choice for critical domains where understanding is important such as in medical fields, finance, etc; (iv) can provide an approximated confidence region for the missing values in a given sample; (v) suitable for both small and large scale data; (vi) in many scenarios, does not require a huge number of parameters as deep learning approaches; (vii) handle multicollinearity in imputation effectively; and (viii) is robust to the normally distributed assumption that its theoretical grounds rely on.

==> formated_algos/algo2.tex <==
% \begin{algorithm}[tb]
%     \caption[dimv]{DIMV algorithm}
%     \label{alg:dimf}

%     \begin{algorithmic}
%         \STATE {\bfseries Input:} \textbf{\textit{centered}} training samples $\mathcal{X}_{train}$, \textbf{\textit{centered}} test samples $\mathcal{X}_{test}$, feature $f$ with missing value

%         \STATE $\hat{\mu}, \hat{\mathbf{\Sigma}} \leftarrow \text{DPER*}(\mathcal{X}_{train})$
%         \FOR {feature $f$ with missing value}
%             \STATE the column in $\mathcal{X}_{test}$ corresponding to $f \leftarrow$ \texttt{DIMV1feature}$(\mathcal{X}_{train}, \mathcal{X}_{test}, f, \alpha, \hat{\mathbf{\Sigma}})$
%         \ENDFOR
%         \STATE \textbf{return} Imputed $\mathcal{X}_{test}$.
%     \end{algorithmic}

% \end{algorithm}

==> formated_algos/dataset_des.tex <==
\begin{table}[ht]
    \caption{Description of datasets used in the experiment} 
    
    \label{tab-datasets}
    \vskip 0.15in
    \begin{center}
    \begin{small}
    \begin{sc}
    \begin{tabular}{lccccr}
        \toprule
        Dataset  &  \#Class & \#Features & \#Sample  \\
        \midrule
        % Iris          &  3     & 4    &  150 \\
        % Thyroid  & 3    &  5   &  215 \\ 
        % Yeast         &  10    & 8    &   1484\\ 
        MNIST         &  10    &  784 & 70000  \\ 
        Fashion-MNIST &  10    &  784 & 70000   \\ 
        Parkinson & 2 & 754 & 756\\
        Spam & 2 & 58 & 4601\\
        \bottomrule
    \end{tabular}
    \end{sc}
    \end{small}
    \end{center}
    \vskip -0.1in
\end{table}   


==> formated_algos/dataset_nips.tex <==
\begin{table}[ht]
    \caption{Description of datasets used in the experiment}  
    \label{tab-datasets}
    \vskip 0.15in
    \begin{center}
    \begin{small}
    \begin{sc}
    \begin{tabular}{lccccr}
        \toprule
        Dataset  & \#Features & \#Sample  \ #Missing type\\
        \midrule
        % Iris          &  3     & 4    &  150 \\
        % Thyroid  & 3    &  5   &  215 \\ 
        % Yeast         &  10    & 8    &   1484\\ 
        MNIST              &  784 & 70000 & Monotone Missing \\ 
        Fashion-MNIST      &  784 & 70000 & Monotone Missing  \\ 
        Yeast    &  8  & 1484 & Randomly Missing  \\
        Thyroid  &  5  & 215  & Randomly Missing  \\ 
        Seeds    &  7  & 210 & Randomly Missing   \\ 
        Iris     &  4  & 150  & Randomly Missing \\ 
        \bottomrule
    \end{tabular}
    \end{sc}
    \end{small}
    \end{center}
    \vskip -0.1in
\end{table}   
 

==> formated_algos/dpers.tex <==
\begin{algorithm}
    \caption[dper*]{$\text{DPER}^*$}
    \label{alg:dpers}
    \begin{algorithmic}[tb]
        \STATE {\bfseries Input: } a \textbf{\textit{centered}} dataset of $p$ features $X \in \mathbb{R}^{n \times p}$,

        \STATE {\bfseries Output:} $\hat{\boldsymbol {\mu }}, \hat{\mathbf{\Sigma}} = (\hat{\sigma}_{ij})_{i,j=1}^p$,

        \STATE {\bfseries Procedure:}

        \STATE $\hat{\boldsymbol {\mu }} \leftarrow 0$

        \STATE Estimate the diagonal elements of $\mathbf{\hat\Sigma}$: $\hat{\sigma}_{ii}$ is the uncorrected sample variance of all the available entries in the $i^{th}$ feature.
        % \STATE $\mathbf{\Sigma} \leftarrow \text{Diag}{[(\hat{\sigma}_{ii})_{ i=1\dots p}]}$. In which, $\hat\sigma_{ii} = \text{Var}(X^{(i)})$

        \FOR {$\hat{\sigma}_{ij}$ entry lies below the diagonal of $\mathbf{\hat\Sigma}$}
            \STATE Compute $\hat{\sigma}_{ij}$ based on Equation  (\ref{der01}). If there are two solutions maximizing the function, choose the one closest to the estimate based on case deletion.
        \ENDFOR

        \STATE $\hat{\mathbf{\Sigma}} \leftarrow \frac{1}{2}(\hat{\mathbf{\Sigma}} + \hat{\mathbf{\Sigma}}^T)$

        \STATE $\text{Diag }(\hat{\mathbf{\Sigma}}) \leftarrow \text{Diag }(\hat{\mathbf{\Sigma}}) /2$

        \STATE \textbf{return} $\hat{\boldsymbol {\mu }}, \hat{\mathbf{\Sigma}}$
     \end{algorithmic}
\end{algorithm}

==> formated_algos/table_5.2.2.1.tex <==
% \begin{table*}[t]
%     \caption{Classification results on imputed data}
%     \label{sample-table}
%     \vskip 0.15in
%     \begin{center}
%     \begin{small}
%     \begin{sc}
%     \begin{tabular}{lccccccccr}
%     \toprule
% dataset     & missing rate  & DIMV                           & imputePCA                     & kNNimpute             & mice                          & missForest                    &  softImpute                   \\
%     \midrule
%             & 10\%          & 94.0\% $\pm$ 3.6\%              & 90.7\% $\pm$ 6.2\%            & 94.0\% $\pm$ 4.5\%    & 92.7\% $\pm$ 4.5\%            & 94.0\% $\pm$ 4.5\%            & \textbf{94.7\% $\pm$ 3.8\%}   \\
%             & 20\%          & \textbf{93.3\% $\pm$ 3.4\%}     & 90.7\% $\pm$ 3.5\%            & 83.3\% $\pm$ 4.5\%    & 92.0\% $\pm$ 3.3\%            & 92.0\% $\pm$ 4.3\%            & \textbf{93.3\% $\pm$ 3.4\%}   \\
% Iris        & 30\%          & 92.0\% $\pm$ 3.3\%              & 89.3\% $\pm$ 2.9\%            & 87.3\% $\pm$ 7.1\%    & \textbf{93.3\% $\pm$ 3.4\%}   & \textbf{93.3\% $\pm$ 3.4\%}   & 88.7\% $\pm$ 4.8\%            \\
%             & 40\%          & \textbf{92.0\% $\pm$ 5.4\%}     & 84.0\% $\pm$ 3.5\%            & 84.0\% $\pm$ 4.0\%    & 86.7\% $\pm$ 2.8\%            & 90.0\% $\pm$ 4.5\%            & 88.7\% $\pm$ 4.4\%            \\
%             & 50\%          & \textbf{88.7\% $\pm$ 3.9\%}     & 77.3\% $\pm$ 6.5\%            & 78.0\% $\pm$ 5.9\%    & 83.3\% $\pm$ 7.4\%            & 85.3\% $\pm$ 6.1\%            & 83.3\% $\pm$ 8.1\%            \\ 
%             \hline
%             & 10\%          & 93.9\% $\pm$ 3.4\%              & \textbf{94.9\% $\pm$ 3.5\%}   & 93.4\% $\pm$ 3.2\%    & 93.5\% $\pm$ 2.5\%            & 93.9\% $\pm$ 3.1\%            & 90.7\% $\pm$ 5.4\%            \\
%             & 20\%          & \textbf{94.0\% $\pm$ 2.4\%}     & 92.6\% $\pm$ 3.0\%            & 91.6\% $\pm$ 3.5\%    & 93.5\% $\pm$ 2.8\%            & 92.6\% $\pm$ 5.0\%            & 83.2\% $\pm$ 3.2\%            \\
% New Thyroid & 30\%          & 91.2\% $\pm$ 4.5\%              & 92.2\% $\pm$ 4.4\%            & 87.6\% $\pm$ 4.9\%    & 89.0\% $\pm$ 4.4\%            & \textbf{92.6\% $\pm$ 4.4\%}   & 80.0\% $\pm$ 4.8\%            \\
%             & 40\%          & 87.5\% $\pm$ 4.0\%              & 85.6\% $\pm$ 5.5\%            & 82.8\% $\pm$ 3.6\%    & 79.5\% $\pm$ 5.6\%            & \textbf{88.8\% $\pm$ 3.7\%}   & 73.1\% $\pm$ 9.6\%            \\
%             & 50\%          & \textbf{87.9\% $\pm$ 4.4\%}     & 82.8\% $\pm$ 3.2\%            & 79.1\% $\pm$ 4.4\%    & 80.1\% $\pm$ 4.6\%            & 87.0\% $\pm$ 3.2\%            & 71.2\% $\pm$ 5.6\%            \\
%             \hline
%             & 10\%          & 91.0\% $\pm$ 5.5\%              & 92.9\% $\pm$ 3.7\%            & 91.4\% $\pm$ 7.1\%    & \textbf{93.3\% $\pm$ 4.2\%}   & \textbf{93.3\% $\pm$ 4.7\%}   & \textbf{93.3\% $\pm$ 4.0\%}   \\
%             & 20\%          & 91.0\% $\pm$ 4.0\%              & 90.5\% $\pm$ 3.9\%            & 87.1\% $\pm$ 5.2\%    & \textbf{93.3\% $\pm$ 4.0\%}   & 91.0\% $\pm$ 4.0\%            & 90.5\% $\pm$ 4.6\%            \\
% Seeds       & 30\%          & 86.2\% $\pm$ 4.9\%              & \textbf{89.0\% $\pm$ 5.0\%}   & 79.5\% $\pm$ 3.9\%    & 86.7\% $\pm$ 8.8\%            & 88.1\% $\pm$ 5.9\%            & 86.2\% $\pm$ 6.1\%            \\
%             & 40\%          & 88.6\% $\pm$ 4.2\%              & 85.2\% $\pm$ 4.9\%            & 75.7\% $\pm$ 7.8\%    & 87.1\% $\pm$ 3.1\%            & \textbf{90.0\% $\pm$ 3.5\%}   & 83.8\% $\pm$ 5.2\%            \\
%             & 50\%          & 81.0\% $\pm$ 5.7\%              & 79.0\% $\pm$ 6.8\%            & 63.8\% $\pm$ 7.0\%    & 81.4\% $\pm$ 4.7\%            & \textbf{86.2\% $\pm$ 4.5\%}   & 79.0\% $\pm$ 7.1\%            \\
%     \bottomrule
%     \end{tabular}
%     \end{sc}
%     \end{small}
%     \end{center}
%     \vskip -0.1in
%     \end{table*}



% \begin{table*}[t]
%     \caption{RMSE results of imputed data}
%     \setlength{\tabcolsep}{1.4 pt}
%     \label{sample-table}
%     \vskip 0.15in
%     \begin{center}
%     \begin{small}
%     \begin{sc}
% \begin{tabular}{lccccccccr}
% \toprule
%     dataset & missing rate &                     dimv &             Gain &                imputePCA &        kNNimpute &            mice &               missForest &       ALS \\
% \midrule
%        iris &     $ 10\% $ &          0.35$\pm$0.09 &  1.97$\pm$0.62 &          0.69$\pm$0.22 &  0.63$\pm$0.32 & 0.43$\pm$0.18 & \textbf{0.31$\pm$0.11} &  0.52$\pm$0.06 \\
%        iris &     $ 20\% $ & \textbf{0.33$\pm$0.11} &   2.22$\pm$0.3 &          0.58$\pm$0.13 &   0.7$\pm$0.14 & 0.63$\pm$0.28 &          0.34$\pm$0.21 &  0.82$\pm$0.43 \\
%        iris &     $ 30\% $ &          0.44$\pm$0.07 &  1.18$\pm$0.21 &          0.74$\pm$0.07 &  0.71$\pm$0.15 & 0.58$\pm$0.17 & \textbf{0.38$\pm$0.08} &   0.65$\pm$0.2 \\
%        iris &     $ 40\% $ &          0.47$\pm$0.08 &  2.22$\pm$0.25 &          0.74$\pm$0.08 &  0.88$\pm$0.23 & 0.63$\pm$0.13 & \textbf{0.45$\pm$0.17} &  0.84$\pm$0.31 \\
%        iris &     $ 50\% $ &           0.61$\pm$0.1 &  2.18$\pm$0.11 &          0.82$\pm$0.09 &   1.0$\pm$0.16 & 0.79$\pm$0.12 & \textbf{0.58$\pm$0.16} &  0.95$\pm$0.19 \\
% \midrule
% new thyroid &     $ 10\% $ &          6.81$\pm$2.61 & 50.27$\pm$8.44 &           6.99$\pm$2.7 & 10.01$\pm$3.71 &  7.06$\pm$2.5 & \textbf{6.26$\pm$2.39} & 10.58$\pm$3.45 \\
% new thyroid &     $ 20\% $ &          4.84$\pm$1.37 & 50.95$\pm$6.75 & \textbf{4.21$\pm$1.42} &  5.66$\pm$1.37 &  6.9$\pm$2.75 &          4.86$\pm$1.04 &  12.03$\pm$4.0 \\
% new thyroid &     $ 30\% $ &          6.62$\pm$1.19 & 56.53$\pm$6.36 &          6.28$\pm$1.11 &  8.33$\pm$1.67 & 7.96$\pm$1.25 & \textbf{5.09$\pm$1.02} & 16.68$\pm$6.76 \\
% new thyroid &     $ 40\% $ &          6.54$\pm$1.12 & 53.72$\pm$4.45 &          6.62$\pm$1.08 &  9.43$\pm$1.13 & 8.27$\pm$2.07 & \textbf{6.49$\pm$1.48} & 16.34$\pm$4.98 \\
% new thyroid &     $ 50\% $ &          7.85$\pm$1.21 & 57.53$\pm$3.52 &          8.39$\pm$1.26 &  10.7$\pm$1.36 & 9.16$\pm$0.89 &  
% \textbf{7.52$\pm$0.9} & 12.91$\pm$3.53 \\
% \midrule
%       yeast &     $ 10\% $ &           0.1$\pm$0.01 &  0.26$\pm$0.01 &           0.1$\pm$0.01 &  0.13$\pm$0.01 & 0.13$\pm$0.02 & \textbf{0.09$\pm$0.01} &  0.26$\pm$0.08 \\
%       yeast &     $ 20\% $ &  \textbf{0.1$\pm$0.01} &  0.26$\pm$0.01 &           0.1$\pm$0.01 &  0.13$\pm$0.01 & 0.13$\pm$0.01 &           0.1$\pm$0.01 &  0.18$\pm$0.03 \\
%       yeast &     $ 30\% $ &  \textbf{0.1$\pm$0.01} &  0.27$\pm$0.01 &           0.1$\pm$0.01 &   0.13$\pm$0.0 &  0.14$\pm$0.0 &           0.1$\pm$0.01 &  0.27$\pm$0.07 \\
%       yeast &     $ 40\% $ &  \textbf{0.1$\pm$0.01} &  0.26$\pm$0.01 &           0.1$\pm$0.01 &  0.13$\pm$0.01 & 0.13$\pm$0.01 &           0.1$\pm$0.01 &  0.23$\pm$0.03 \\
%       yeast &     $ 50\% $ &  \textbf{0.09$\pm$0.0} &  0.26$\pm$0.01 &            0.1$\pm$0.0 &   0.12$\pm$0.0 & 0.14$\pm$0.01 &            0.1$\pm$0.0 &  0.29$\pm$0.05 \\
% \bottomrule
% \end{tabular}
% \end{sc}
% \end{small}
% \end{center}
% \vskip -0.1in
% \end{table*}




% \begin{table*}[t]
%     \caption{RMSE results of imputed data}
%     \setlength{\tabcolsep}{1.5 pt}
%     \label{sample-table}
%     \vskip 0.15in
%     \begin{center}
%     \begin{small}
%     \begin{sc}
% \begin{tabular}{lccccccccr}
% \toprule
%     dataset & missing rate &                   DIMV &               imputePCA &      kNNimpute &                    mice &             softImpute &                    Gain &                    GINN \\
% \midrule
%         &     $ 10\% $ &   \textbf{0.30$\pm$0.07} &        0.59$\pm$0.15 &   0.73$\pm$0.45 &   0.43$\pm$0.09 &   0.46$\pm$0.05 &   0.64$\pm$0.28 &          0.81$\pm$0.26 \\
%         &     $ 20\% $ &   \textbf{0.35$\pm$0.05} &        0.65$\pm$0.06 &   0.72$\pm$0.23 &   0.50$\pm$0.14 &   0.48$\pm$0.09 &   0.69$\pm$0.13 &          1.00$\pm$0.06 \\
%        iris &     $ 30\% $ &   \textbf{0.51$\pm$0.13} &        0.57$\pm$0.07 &   0.73$\pm$0.14 &   0.62$\pm$0.16 &   0.71$\pm$0.43 &   0.64$\pm$0.14 &          0.88$\pm$0.08 \\
%         &     $ 40\% $ &   \textbf{0.48$\pm$0.14} &        0.76$\pm$0.11 &   0.94$\pm$0.28 &   0.75$\pm$0.19 &   1.17$\pm$1.00 &   0.79$\pm$0.22 &          0.95$\pm$0.10 \\
%         &     $ 50\% $ &   \textbf{0.63$\pm$0.11} &        0.83$\pm$0.06 &   1.09$\pm$0.15 &   0.80$\pm$0.14 &   0.72$\pm$0.12 &   1.03$\pm$0.28 &          0.97$\pm$0.10 \\
%        \midrule
% &     $ 10\% $ &   \textbf{5.88$\pm$2.51} &         6.0$\pm$2.85 &   7.27$\pm$2.49 &   6.02$\pm$3.07 & 16.22$\pm$14.71 &   7.19$\pm$2.79 &          6.15$\pm$2.92 \\
%  &     $ 20\% $ &    \textbf{7.63$\pm$1.30} &        7.67$\pm$1.64 &   9.89$\pm$1.96 &   9.37$\pm$1.79 &  13.22$\pm$4.25 &    8.8$\pm$2.24 &           8.46$\pm$1.50 \\
% thyroid &     $ 30\% $ &            7.81$\pm$1.25 &        7.84$\pm$1.08 &     9.1$\pm$1.5 &   8.98$\pm$1.19 &   13.77$\pm$5.30 &   8.52$\pm$2.07 &  \textbf{7.6$\pm$1.21} \\
%  &     $ 40\% $ &            6.74$\pm$1.21 & \textbf{6.60$\pm$1.10} &   7.66$\pm$2.06 &    8.22$\pm$1.80 &  12.32$\pm$3.77 &   8.76$\pm$1.41 &          6.63$\pm$0.81 \\
%  &     $ 50\% $ &           10.23$\pm$6.39 &        6.88$\pm$0.77 &   8.22$\pm$1.13 &   8.89$\pm$0.49 &  14.99$\pm$4.47 &  10.46$\pm$2.25 & \textbf{6.78$\pm$0.68} \\
% \midrule 
%  &     $ 10\% $ & \textbf{0.087$\pm$0.009} &      0.091$\pm$0.008 & 0.121$\pm$0.014 & 0.129$\pm$0.009 & 0.145$\pm$0.044 &  0.098$\pm$0.01 &        0.092$\pm$0.008 \\
%        &     $ 20\% $ & \textbf{0.099$\pm$0.004} &        0.1$\pm$0.005 & 0.127$\pm$0.008 & 0.142$\pm$0.005 & 0.191$\pm$0.073 &  0.12$\pm$0.008 &        0.102$\pm$0.004 \\
%       yeast &     $ 30\% $ & \textbf{0.094$\pm$0.002} &      0.097$\pm$0.001 & 0.126$\pm$0.001 & 0.132$\pm$0.006 & 0.209$\pm$0.012 & 0.109$\pm$0.005 &          0.100$\pm$0.001 \\
%        &     $ 40\% $ & \textbf{0.099$\pm$0.006} &      0.103$\pm$0.005 & 0.131$\pm$0.004 & 0.138$\pm$0.004 & 0.206$\pm$0.062 & 0.112$\pm$0.005 &        0.104$\pm$0.005 \\
%        &     $ 50\% $ & \textbf{0.094$\pm$0.003} &      0.097$\pm$0.003 & 0.127$\pm$0.005 & 0.136$\pm$0.004 & 0.211$\pm$0.023 &  0.120$\pm$0.006 &          0.100$\pm$0.004 \\
% \bottomrule
% \end{tabular}
% \end{sc}
% \end{small}
% \end{center}
% \label{rmse-on-randomly-missing-dataset}
% \vskip -0.1in
% \end{table*}
%----------------------------------------------------------------------------------- 
% \begin{table*}[ht]
%     \caption{RMSE results of imputed data}
%     \setlength{\tabcolsep}{1.5 pt}
%     \label{sample-table}
%     \vskip 0.15in
%     \begin{center}
%     \begin{small}
%     \begin{sc}
% \begin{tabular}{lccccccccr}
% \toprule
%     dataset & missing rate &                    DIMV &            imputePCA &       KNNI &            mice &      ALS &            GAIN &                   GINN \\
% \midrule
%         &     $ 10\% $ &    \textbf{0.3$\pm$0.07} &        0.59$\pm$0.15 &   0.73$\pm$0.45 &   0.43$\pm$0.09 &   0.46$\pm$0.05 &   0.64$\pm$a0.28 &          0.81$\pm$0.26 \\
%         &     $ 20\% $ &   \textbf{0.35$\pm$0.05} &        0.65$\pm$0.06 &   0.72$\pm$0.23 &    0.5$\pm$0.14 &   0.48$\pm$0.09 &   0.69$\pm$0.13 &           1.0$\pm$0.06 \\
%        iris &     $ 30\% $ &    \textbf{0.5$\pm$0.14} &        0.57$\pm$0.07 &   0.73$\pm$0.14 &   0.62$\pm$0.16 &   0.71$\pm$0.43 &   0.64$\pm$0.14 &          0.88$\pm$0.08 \\
%         &     $ 40\% $ &   \textbf{0.48$\pm$0.14} &        0.76$\pm$0.11 &   0.94$\pm$0.28 &   0.75$\pm$0.19 &    1.17$\pm$1.0 &   0.79$\pm$0.22 &           0.95$\pm$0.1 \\
%         &     $ 50\% $ &   \textbf{0.63$\pm$0.11} &        0.83$\pm$0.06 &   1.09$\pm$0.15 &    0.8$\pm$0.14 &   0.72$\pm$0.12 &   1.03$\pm$0.28 &           0.97$\pm$0.1 \\
% \midrule
%  &     $ 10\% $ &   \textbf{5.88$\pm$2.51} &         6.0$\pm$2.85 &   7.27$\pm$2.49 &   6.02$\pm$3.07 & 16.22$\pm$14.71 &   7.19$\pm$2.79 &          6.15$\pm$2.92 \\
%  &     $ 20\% $ &    \textbf{7.63$\pm$1.3} &        7.67$\pm$1.64 &   9.89$\pm$1.96 &   9.37$\pm$1.79 &  13.22$\pm$4.25 &    8.8$\pm$2.24 &           8.46$\pm$1.5 \\
% thyroid &     $ 30\% $ &            7.81$\pm$1.25 &        7.84$\pm$1.08 &     9.1$\pm$1.5 &   8.98$\pm$1.19 &   13.77$\pm$5.3 &   8.52$\pm$2.07 &  \textbf{7.6$\pm$1.21} \\
%  &     $ 40\% $ &            6.74$\pm$1.21 & \textbf{6.6$\pm$1.1} &   7.66$\pm$2.06 &    8.22$\pm$1.8 &  12.32$\pm$3.77 &   8.76$\pm$1.41 &          6.63$\pm$0.81 \\
%  &     $ 50\% $ &           10.09$\pm$6.46 &        6.88$\pm$0.77 &   8.22$\pm$1.13 &   8.89$\pm$0.49 &  14.99$\pm$4.47 &  10.46$\pm$2.25 & \textbf{6.78$\pm$0.68} \\
% \midrule
%        &     $ 10\% $ & \textbf{0.087$\pm$0.009} &      0.091$\pm$0.008 & 0.121$\pm$0.014 & 0.129$\pm$0.009 & 0.145$\pm$0.044 &  0.098$\pm$0.01 &        0.092$\pm$0.008 \\
%        &     $ 20\% $ & \textbf{0.099$\pm$0.004} &        0.1$\pm$0.005 & 0.127$\pm$0.008 & 0.142$\pm$0.005 & 0.191$\pm$0.073 &  0.12$\pm$0.008 &        0.102$\pm$0.004 \\
%       yeast &     $ 30\% $ & \textbf{0.095$\pm$0.002} &      0.097$\pm$0.001 & 0.126$\pm$0.001 & 0.132$\pm$0.006 & 0.209$\pm$0.012 & 0.109$\pm$0.005 &          0.1$\pm$0.001 \\
%        &     $ 40\% $ & \textbf{0.099$\pm$0.006} &      0.103$\pm$0.005 & 0.131$\pm$0.004 & 0.138$\pm$0.004 & 0.206$\pm$0.062 & 0.112$\pm$0.005 &        0.104$\pm$0.005 \\
%        &     $ 50\% $ & \textbf{0.094$\pm$0.003} &      0.097$\pm$0.003 & 0.127$\pm$0.005 & 0.136$\pm$0.004 & 0.211$\pm$0.023 &  0.12$\pm$0.006 &          0.1$\pm$0.004 \\
% \bottomrule
% \end{tabular}
% \end{sc}
% \end{small}
% \end{center}
% \label{tab-rmse-on-randomly-missing-dataset}
% \vskip -0.1in
% \end{table*}


%----------------------------------------------------------------------------------- 


\begin{table}[h!]
    \caption{RMSE results of imputed data}
    \setlength{\tabcolsep}{1.5 pt}
    % \label{tab-rmse-on-randomly-missing-dataset}
    \vskip 0.15in
    \begin{center}
    \begin{small}
    \begin{sc}
\begin{tabular}{lccccccccr}
\toprule
    dataset & missing rate &                    DIMV &            imputePCA &       KNNI &            mice &      ALS &            GAIN &                   GINN \\
\midrule
        &     $ 10\% $ &             0.3$\pm$0.07 &   0.59$\pm$0.15 &   0.73$\pm$0.45 &   0.43$\pm$0.09 &   0.46$\pm$0.05 &   0.64$\pm$0.28 &          0.81$\pm$0.26 \\
        &     $ 20\% $ &            0.35$\pm$0.05 &   0.65$\pm$0.06 &   0.72$\pm$0.23 &    0.5$\pm$0.14 &   0.48$\pm$0.09 &   0.69$\pm$0.13 &           1.0$\pm$0.06 \\
       iris &     $ 30\% $ &             0.5$\pm$0.14 &   0.57$\pm$0.07 &   0.73$\pm$0.14 &   0.62$\pm$0.16 &   0.71$\pm$0.43 &   0.64$\pm$0.14 &          0.88$\pm$0.08 \\
        &     $ 40\% $ &   \textbf{0.48$\pm$0.14} &   0.76$\pm$0.11 &   0.94$\pm$0.28 &   0.75$\pm$0.19 &    1.17$\pm$1.0 &   0.79$\pm$0.22 &           0.95$\pm$0.1 \\
        &     $ 50\% $ &            0.63$\pm$0.11 &   0.83$\pm$0.06 &   1.09$\pm$0.15 &    0.8$\pm$0.14 &   0.72$\pm$0.12 &   1.03$\pm$0.28 &           0.97$\pm$0.1 \\
        
 \midrule  
 
 
 &     $ 10\% $ &            5.88$\pm$2.51 &    6.0$\pm$2.85 &   7.27$\pm$2.49 &   6.02$\pm$3.07 & 16.22$\pm$14.71 &   7.19$\pm$2.79 &          6.15$\pm$2.92 \\
 &     $ 20\% $ &             7.63$\pm$1.3 &   7.67$\pm$1.64 &   9.89$\pm$1.96 &   9.37$\pm$1.79 &  13.22$\pm$4.25 &    8.8$\pm$2.24 &           8.46$\pm$1.5 \\
thyroid &     $ 30\% $ &            7.81$\pm$1.25 &   7.84$\pm$1.08 &     9.1$\pm$1.5 &   8.98$\pm$1.19 &   13.77$\pm$5.3 &   8.52$\pm$2.07 &           7.6$\pm$1.21 \\
 &     $ 40\% $ &            6.74$\pm$1.21 &     6.6$\pm$1.1 &   7.66$\pm$2.06 &    8.22$\pm$1.8 &  12.32$\pm$3.77 &   8.76$\pm$1.41 &          6.63$\pm$0.81 \\
 &     $ 50\% $ &           10.09$\pm$6.46 &   6.88$\pm$0.77 &   8.22$\pm$1.13 &   8.89$\pm$0.49 &  14.99$\pm$4.47 &  10.46$\pm$2.25 & \textbf{6.78$\pm$0.68} \\
 
 
  \midrule  
       &     $ 10\% $ &          0.087$\pm$0.009 & 0.091$\pm$0.008 & 0.121$\pm$0.014 & 0.129$\pm$0.009 & 0.145$\pm$0.044 &  0.098$\pm$0.01 &        0.092$\pm$0.008 \\
       &     $ 20\% $ & \textbf{0.099$\pm$0.004} &   0.1$\pm$0.005 & 0.127$\pm$0.008 & 0.142$\pm$0.005 & 0.191$\pm$0.073 &  0.12$\pm$0.008 &        0.102$\pm$0.004 \\
      yeast &     $ 30\% $ & \textbf{0.095$\pm$0.002} & 0.097$\pm$0.001 & 0.126$\pm$0.001 & 0.132$\pm$0.006 & 0.209$\pm$0.012 & 0.109$\pm$0.005 &          0.1$\pm$0.001 \\
       &     $ 40\% $ & \textbf{0.099$\pm$0.006} & 0.103$\pm$0.005 & 0.131$\pm$0.004 & 0.138$\pm$0.004 & 0.206$\pm$0.062 & 0.112$\pm$0.005 &        0.104$\pm$0.005 \\
       &     $ 50\% $ & \textbf{0.094$\pm$0.003} & 0.097$\pm$0.003 & 0.127$\pm$0.005 & 0.136$\pm$0.004 & 0.211$\pm$0.023 &  0.12$\pm$0.006 &          0.1$\pm$0.004 \\
\bottomrule
\end{tabular}
\end{sc}
\end{small}
\end{center}
\label{tab-rmse-tabular}
\vskip -0.1in
\end{table} 

==> formated_algos/table_5.2.2.1_extra.tex <==
\begin{table*}[ht]
    \caption{RMSE results of imputed data}
    \setlength{\tabcolsep}{1.5 pt}
    \label{tab-rmse-tabular2}
    \vskip 0.15in
    \begin{center}
    \begin{small}
    \begin{sc}
\begin{tabular}{lcccr}
\toprule
    dataset & missing rate &               missForest &              EM &         MeanImp \\
\midrule
        &     $ 10\% $ &   \textbf{0.29$\pm$0.08} &   0.38$\pm$0.08 &   0.99$\pm$0.25 \\
        &     $ 20\% $ &   \textbf{0.31$\pm$0.06} &   0.54$\pm$0.22 &   1.15$\pm$0.08 \\
       iris &     $ 30\% $ &   \textbf{0.43$\pm$0.12} &   0.53$\pm$0.09 &    1.0$\pm$0.09 \\
        &     $ 40\% $ &            0.52$\pm$0.13 &   0.59$\pm$0.09 &   1.07$\pm$0.07 \\
        &     $ 50\% $ &    \textbf{0.62$\pm$0.2} &   0.72$\pm$0.14 &   1.05$\pm$0.09 \\
\midrule        
        
 &     $ 10\% $ &    \textbf{4.64$\pm$2.0} &  10.75$\pm$4.16 &   6.33$\pm$3.35 \\
 &     $ 20\% $ &   \textbf{6.96$\pm$1.65} &   9.55$\pm$2.58 &    9.2$\pm$1.75 \\
thyroid &     $ 30\% $ &   \textbf{6.04$\pm$0.85} &   10.3$\pm$1.01 &    8.17$\pm$1.2 \\
 &     $ 40\% $ &    \textbf{6.4$\pm$1.35} &  10.55$\pm$4.43 &   6.99$\pm$0.93 \\
 &     $ 50\% $ &            6.94$\pm$0.68 &   11.4$\pm$2.37 &   7.05$\pm$0.75 \\
\midrule 
 
       &     $ 10\% $ & \textbf{0.086$\pm$0.009} & 0.126$\pm$0.004 & 0.097$\pm$0.008 \\
       &     $ 20\% $ &          0.101$\pm$0.004 & 0.133$\pm$0.002 & 0.106$\pm$0.004 \\
      yeast &     $ 30\% $ &          0.098$\pm$0.002 & 0.133$\pm$0.003 & 0.101$\pm$0.001 \\
       &     $ 40\% $ &          0.106$\pm$0.008 & 0.139$\pm$0.005 & 0.104$\pm$0.005 \\
       &     $ 50\% $ &          0.107$\pm$0.002 & 0.138$\pm$0.003 & 0.098$\pm$0.004 \\
\bottomrule
\end{tabular}
\end{sc}
\end{small}
\end{center}
\label{tab-rmse-on-randomly-missing-dataset}
\vskip -0.1in
\end{table*}

==> formated_algos/table_5.2.2.1_extra_v2.tex <==
\begin{table*}[ht]
    \caption{RMSE results of imputed data}
    \setlength{\tabcolsep}{1.5 pt}
    \label{tab-rmse-tabular2}
    \vskip 0.15in
    \begin{center}
    \begin{small}
    \begin{sc}
\begin{tabular}{lcccr}
\toprule
    dataset & missing rate &               missForest &              EM &         MeanImp \\
    \midrule
        &     $ 10\% $ &   \textbf{0.29$\pm$0.08} &   0.38$\pm$0.08 &    1.0$\pm$0.26 \\
        &     $ 20\% $ &   \textbf{0.31$\pm$0.06} &   0.54$\pm$0.22 &   1.15$\pm$0.11 \\
       iris &     $ 30\% $ &   \textbf{0.43$\pm$0.12} &   0.53$\pm$0.09 &   1.02$\pm$0.07 \\
        &     $ 40\% $ &            0.52$\pm$0.13 &   0.59$\pm$0.09 &   1.07$\pm$0.07 \\
        &     $ 50\% $ &    \textbf{0.62$\pm$0.2} &   0.72$\pm$0.14 &   1.06$\pm$0.08 \\
\midrule
 &     $ 10\% $ &    \textbf{4.64$\pm$2.0} &  10.75$\pm$4.16 &   6.51$\pm$3.36 \\
 &     $ 20\% $ &   \textbf{6.96$\pm$1.65} &   9.55$\pm$2.58 &   9.25$\pm$1.91 \\
thyroid &     $ 30\% $ &   \textbf{6.04$\pm$0.85} &   10.3$\pm$1.01 &   8.44$\pm$1.18 \\
 &     $ 40\% $ &    \textbf{6.4$\pm$1.35} &  10.55$\pm$4.43 &   7.14$\pm$0.89 \\
 &     $ 50\% $ &            6.94$\pm$0.68 &   11.4$\pm$2.37 &   7.37$\pm$0.98 \\
\midrule
       &     $ 10\% $ & \textbf{0.086$\pm$0.009} & 0.126$\pm$0.004 & 0.097$\pm$0.008 \\
       &     $ 20\% $ &          0.101$\pm$0.004 & 0.133$\pm$0.002 & 0.106$\pm$0.005 \\
      yeast &     $ 30\% $ &          0.098$\pm$0.002 & 0.133$\pm$0.003 & 0.102$\pm$0.001 \\
       &     $ 40\% $ &          0.106$\pm$0.008 & 0.139$\pm$0.005 & 0.104$\pm$0.005 \\
       &     $ 50\% $ &          0.107$\pm$0.002 & 0.138$\pm$0.003 & 0.098$\pm$0.004 \\
\bottomrule
\end{tabular}
\end{sc}
\end{small}
\end{center}
%\label{tab-rmse-on-randomly-missing-dataset}
\vskip -0.1in
\end{table*}

==> formated_algos/table_5.2.2.1_v2.tex <==

\begin{table}[h!]
    \caption{RMSE results of imputed data}
    \setlength{\tabcolsep}{1.5 pt}
    % \label{sample-table}
    \vskip 0.15in
    \begin{center}
    \begin{small}
    \begin{sc}
\begin{tabular}{lccccccccr}
\toprule
    dataset & missing rate &                    DIMV &            imputePCA &       KNNI &            mice &      ALS &            GAIN &                   GINN \\
\midrule
 &     $ 10\% $ &             0.3$\pm$0.07 &   0.59$\pm$0.15 &   0.73$\pm$0.45 &   0.43$\pm$0.09 &   0.46$\pm$0.05 &   0.64$\pm$0.28 &          0.81$\pm$0.26 \\
 &     $ 20\% $ &            0.35$\pm$0.05 &   0.65$\pm$0.06 &   0.72$\pm$0.23 &    0.5$\pm$0.14 &   0.48$\pm$0.09 &   0.69$\pm$0.13 &           1.0$\pm$0.06 \\
iris &     $ 30\% $ &             0.5$\pm$0.14 &   0.57$\pm$0.07 &   0.73$\pm$0.14 &   0.62$\pm$0.16 &   0.71$\pm$0.43 &   0.64$\pm$0.14 &          0.88$\pm$0.08 \\
 &     $ 40\% $ &   \textbf{0.48$\pm$0.14} &   0.76$\pm$0.11 &   0.94$\pm$0.28 &   0.75$\pm$0.19 &    1.17$\pm$1.0 &   0.79$\pm$0.22 &           0.95$\pm$0.1 \\
 &     $ 50\% $ &            0.63$\pm$0.11 &   0.83$\pm$0.06 &   1.09$\pm$0.15 &    0.8$\pm$0.14 &   0.72$\pm$0.12 &   1.03$\pm$0.28 &           0.97$\pm$0.1 \\
\midrule
 &     $ 10\% $ &            5.88$\pm$2.51 &    6.0$\pm$2.85 &   7.27$\pm$2.49 &   6.02$\pm$3.07 & 16.22$\pm$14.71 &   7.19$\pm$2.79 &          6.15$\pm$2.92 \\
 &     $ 20\% $ &             7.63$\pm$1.3 &   7.67$\pm$1.64 &   9.89$\pm$1.96 &   9.37$\pm$1.79 &  13.22$\pm$4.25 &    8.8$\pm$2.24 &           8.46$\pm$1.5 \\
thyroid &     $ 30\% $ &            7.81$\pm$1.25 &   7.84$\pm$1.08 &     9.1$\pm$1.5 &   8.98$\pm$1.19 &   13.77$\pm$5.3 &   8.52$\pm$2.07 &           7.6$\pm$1.21 \\
 &     $ 40\% $ &            6.74$\pm$1.21 &     6.6$\pm$1.1 &   7.66$\pm$2.06 &    8.22$\pm$1.8 &  12.32$\pm$3.77 &   8.76$\pm$1.41 &          6.63$\pm$0.81 \\
 &     $ 50\% $ &           10.09$\pm$6.46 &   6.88$\pm$0.77 &   8.22$\pm$1.13 &   8.89$\pm$0.49 &  14.99$\pm$4.47 &  10.46$\pm$2.25 & \textbf{6.78$\pm$0.68} \\
\midrule
 &     $ 10\% $ &          0.087$\pm$0.009 & 0.091$\pm$0.008 & 0.121$\pm$0.014 & 0.129$\pm$0.009 & 0.145$\pm$0.044 &  0.098$\pm$0.01 &        0.092$\pm$0.008 \\
 &     $ 20\% $ & \textbf{0.099$\pm$0.004} &   0.1$\pm$0.005 & 0.127$\pm$0.008 & 0.142$\pm$0.005 & 0.191$\pm$0.073 &  0.12$\pm$0.008 &        0.102$\pm$0.004 \\
yeast &     $ 30\% $ & \textbf{0.095$\pm$0.002} & 0.097$\pm$0.001 & 0.126$\pm$0.001 & 0.132$\pm$0.006 & 0.209$\pm$0.012 & 0.109$\pm$0.005 &          0.1$\pm$0.001 \\
 &     $ 40\% $ & \textbf{0.099$\pm$0.006} & 0.103$\pm$0.005 & 0.131$\pm$0.004 & 0.138$\pm$0.004 & 0.206$\pm$0.062 & 0.112$\pm$0.005 &        0.104$\pm$0.005 \\
 &     $ 50\% $ & \textbf{0.094$\pm$0.003} & 0.097$\pm$0.003 & 0.127$\pm$0.005 & 0.136$\pm$0.004 & 0.211$\pm$0.023 &  0.12$\pm$0.006 &          0.1$\pm$0.004 \\
\bottomrule
\end{tabular}
\end{sc}
\end{small}
\end{center}
\label{tab-rmse-tabular}
\vskip -0.1in
\end{table} 

==> formated_algos/table_5.2.2.2.tex <==
% \begin{table*}[t]
%     \caption{Classification results on imputed data}
%     \label{sample-table}
%     \vskip 0.15in
%     \begin{center}
%     \begin{small}
%     \begin{sc}
%     \begin{tabular}{lccccccccr}
%     \toprule
% dataset     & missing rate  & DIMV                           & imputePCA                     & kNNimpute             & mice                          & missForest                    &  softImpute                   \\
%     \midrule
%             & 10\%          & 94.0\% $\pm$ 3.6\%              & 90.7\% $\pm$ 6.2\%            & 94.0\% $\pm$ 4.5\%    & 92.7\% $\pm$ 4.5\%            & 94.0\% $\pm$ 4.5\%            & \textbf{94.7\% $\pm$ 3.8\%}   \\
%             & 20\%          & \textbf{93.3\% $\pm$ 3.4\%}     & 90.7\% $\pm$ 3.5\%            & 83.3\% $\pm$ 4.5\%    & 92.0\% $\pm$ 3.3\%            & 92.0\% $\pm$ 4.3\%            & \textbf{93.3\% $\pm$ 3.4\%}   \\
% Iris        & 30\%          & 92.0\% $\pm$ 3.3\%              & 89.3\% $\pm$ 2.9\%            & 87.3\% $\pm$ 7.1\%    & \textbf{93.3\% $\pm$ 3.4\%}   & \textbf{93.3\% $\pm$ 3.4\%}   & 88.7\% $\pm$ 4.8\%            \\
%             & 40\%          & \textbf{92.0\% $\pm$ 5.4\%}     & 84.0\% $\pm$ 3.5\%            & 84.0\% $\pm$ 4.0\%    & 86.7\% $\pm$ 2.8\%            & 90.0\% $\pm$ 4.5\%            & 88.7\% $\pm$ 4.4\%            \\
%             & 50\%          & \textbf{88.7\% $\pm$ 3.9\%}     & 77.3\% $\pm$ 6.5\%            & 78.0\% $\pm$ 5.9\%    & 83.3\% $\pm$ 7.4\%            & 85.3\% $\pm$ 6.1\%            & 83.3\% $\pm$ 8.1\%            \\ 
%             \hline
%             & 10\%          & 93.9\% $\pm$ 3.4\%              & \textbf{94.9\% $\pm$ 3.5\%}   & 93.4\% $\pm$ 3.2\%    & 93.5\% $\pm$ 2.5\%            & 93.9\% $\pm$ 3.1\%            & 90.7\% $\pm$ 5.4\%            \\
%             & 20\%          & \textbf{94.0\% $\pm$ 2.4\%}     & 92.6\% $\pm$ 3.0\%            & 91.6\% $\pm$ 3.5\%    & 93.5\% $\pm$ 2.8\%            & 92.6\% $\pm$ 5.0\%            & 83.2\% $\pm$ 3.2\%            \\
% New Thyroid & 30\%          & 91.2\% $\pm$ 4.5\%              & 92.2\% $\pm$ 4.4\%            & 87.6\% $\pm$ 4.9\%    & 89.0\% $\pm$ 4.4\%            & \textbf{92.6\% $\pm$ 4.4\%}   & 80.0\% $\pm$ 4.8\%            \\
%             & 40\%          & 87.5\% $\pm$ 4.0\%              & 85.6\% $\pm$ 5.5\%            & 82.8\% $\pm$ 3.6\%    & 79.5\% $\pm$ 5.6\%            & \textbf{88.8\% $\pm$ 3.7\%}   & 73.1\% $\pm$ 9.6\%            \\
%             & 50\%          & \textbf{87.9\% $\pm$ 4.4\%}     & 82.8\% $\pm$ 3.2\%            & 79.1\% $\pm$ 4.4\%    & 80.1\% $\pm$ 4.6\%            & 87.0\% $\pm$ 3.2\%            & 71.2\% $\pm$ 5.6\%            \\
%             \hline
%             & 10\%          & 91.0\% $\pm$ 5.5\%              & 92.9\% $\pm$ 3.7\%            & 91.4\% $\pm$ 7.1\%    & \textbf{93.3\% $\pm$ 4.2\%}   & \textbf{93.3\% $\pm$ 4.7\%}   & \textbf{93.3\% $\pm$ 4.0\%}   \\
%             & 20\%          & 91.0\% $\pm$ 4.0\%              & 90.5\% $\pm$ 3.9\%            & 87.1\% $\pm$ 5.2\%    & \textbf{93.3\% $\pm$ 4.0\%}   & 91.0\% $\pm$ 4.0\%            & 90.5\% $\pm$ 4.6\%            \\
% Seeds       & 30\%          & 86.2\% $\pm$ 4.9\%              & \textbf{89.0\% $\pm$ 5.0\%}   & 79.5\% $\pm$ 3.9\%    & 86.7\% $\pm$ 8.8\%            & 88.1\% $\pm$ 5.9\%            & 86.2\% $\pm$ 6.1\%            \\
%             & 40\%          & 88.6\% $\pm$ 4.2\%              & 85.2\% $\pm$ 4.9\%            & 75.7\% $\pm$ 7.8\%    & 87.1\% $\pm$ 3.1\%            & \textbf{90.0\% $\pm$ 3.5\%}   & 83.8\% $\pm$ 5.2\%            \\
%             & 50\%          & 81.0\% $\pm$ 5.7\%              & 79.0\% $\pm$ 6.8\%            & 63.8\% $\pm$ 7.0\%    & 81.4\% $\pm$ 4.7\%            & \textbf{86.2\% $\pm$ 4.5\%}   & 79.0\% $\pm$ 7.1\%            \\
%     \bottomrule
%     \end{tabular}
%     \end{sc}
%     \end{small}
%     \end{center}
%     \vskip -0.1in
%     \end{table*}



% \begin{table*}[t]
%     \caption{Accuracy results on imputed data}
%     \setlength{\tabcolsep}{1.4 pt}
%     \label{sample-table}
%     \vskip 0.15in
%     \begin{center}
%     \begin{small}
%     \begin{sc}
% \begin{tabular}{lccccccccr}
% \toprule
%     dataset & missing rate &                    dimv &            Gain &               imputePCA &               kNNimpute &                    mice &              missForest &     ALS \\
% \midrule
%        iris &     $ 10\% $ &          94.67$\pm$4.27 &  92.67$\pm$4.55 &          91.33$\pm$3.92 &          93.33$\pm$3.37 &           94.67$\pm$3.8 &  \textbf{95.33$\pm$3.4} &  94.0$\pm$4.55 \\
%        iris &     $ 20\% $ &           92.0$\pm$5.08 &   88.67$\pm$7.3 &            92.0$\pm$3.8 &           90.0$\pm$6.24 &           92.0$\pm$5.08 & \textbf{92.67$\pm$5.32} & 91.33$\pm$5.17 \\
%        iris &     $ 30\% $ &          91.33$\pm$4.38 &  82.67$\pm$6.52 &          87.33$\pm$5.99 &          87.33$\pm$5.32 & \textbf{92.67$\pm$4.55} & \textbf{92.67$\pm$4.11} & 86.67$\pm$7.29 \\
%        iris &     $ 40\% $ &          92.67$\pm$4.55 &  80.67$\pm$5.66 &           82.0$\pm$3.92 &          85.33$\pm$5.78 &          88.67$\pm$5.17 & \textbf{93.33$\pm$3.37} & 86.67$\pm$5.51 \\
%        iris &     $ 50\% $ &           84.0$\pm$5.58 &   70.0$\pm$7.09 &           72.0$\pm$5.44 &           84.0$\pm$7.34 &           82.0$\pm$5.86 & \textbf{88.67$\pm$4.79} & 74.0$\pm$10.92 \\
% \midrule
% new thyroid &     $ 10\% $ &          94.91$\pm$2.46 &  89.76$\pm$4.02 & \textbf{95.82$\pm$2.47} &            92.1$\pm$3.8 &          93.51$\pm$2.37 &  
% 94.44$\pm$2.57 & 92.12$\pm$3.78 \\
% new thyroid &     $ 20\% $ &          91.19$\pm$2.06 &   84.74$\pm$6.0 &          92.58$\pm$2.78 &          93.03$\pm$2.41 &          90.28$\pm$3.67 & \textbf{93.51$\pm$3.38} & 82.79$\pm$3.86 \\
% new thyroid &     $ 30\% $ &          87.86$\pm$5.19 &  79.94$\pm$6.62 &          88.77$\pm$4.63 &          84.63$\pm$4.35 &           86.9$\pm$5.77 & \textbf{90.13$\pm$5.13} & 84.13$\pm$3.72 \\
% new thyroid &     $ 40\% $ & \textbf{86.99$\pm$3.29} &  68.44$\pm$5.62 &          85.11$\pm$3.02 &          80.48$\pm$2.64 &          85.04$\pm$6.03 &          86.08$\pm$3.26 & 71.62$\pm$7.47 \\
% new thyroid &     $ 50\% $ & \textbf{87.97$\pm$4.85} & 61.95$\pm$12.62 &          77.64$\pm$5.02 &           78.25$\pm$6.3 &          79.96$\pm$5.24 &          86.54$\pm$3.62 & 72.66$\pm$7.57 \\
%       \midrule
%       yeast &     $ 10\% $ &          56.61$\pm$2.18 &  54.45$\pm$1.76 &           55.6$\pm$2.78 & \textbf{57.08$\pm$2.73} &          55.26$\pm$2.04 &          56.34$\pm$2.49 &  53.98$\pm$3.2 \\
%       yeast &     $ 20\% $ &          52.57$\pm$2.78 &  50.47$\pm$1.88 &          53.04$\pm$2.74 &          51.76$\pm$3.73 &          48.86$\pm$2.93 & \textbf{53.31$\pm$2.53} & 51.48$\pm$2.12 \\
%       yeast &     $ 30\% $ & \textbf{52.35$\pm$3.12} &  44.87$\pm$2.64 &          51.47$\pm$3.17 &          47.03$\pm$2.74 &          46.83$\pm$2.34 &          51.47$\pm$2.46 & 46.89$\pm$2.55 \\
%       yeast &     $ 40\% $ &  \textbf{47.57$\pm$1.5} &  41.71$\pm$1.68 &           47.5$\pm$1.16 &          43.13$\pm$1.39 &          44.88$\pm$1.85 &          46.63$\pm$1.74 & 42.85$\pm$3.39 \\
%       yeast &     $ 50\% $ &  \textbf{44.95$\pm$2.3} &  36.46$\pm$3.22 &          44.35$\pm$2.94 &           40.83$\pm$2.4 &          40.09$\pm$2.73 &          41.85$\pm$2.65 & 37.73$\pm$1.97 \\
% \bottomrule
% \end{tabular}
% \end{sc}
% \end{small}
% \end{center}
% \vskip -0.1in
% \end{table*}


% \begin{table*}[t]
%     \caption{Accuracy results on imputed data}
%     \setlength{\tabcolsep}{1.5 pt}
%     \label{sample-table}
%     \vskip 0.15in
%     \begin{center}
%     \begin{small}
%     \begin{sc}
% \begin{tabular}{lcccccccr}
%     \toprule
%     dataset & missing rate &                   DIMV &               imputePCA &      kNNimpute &                    mice &             softImpute &                    Gain &                    GINN \\
% \midrule
%         &     $ 10\% $ &           95.33$\pm$1.60 &           92.67$\pm$3.2 & 93.33$\pm$2.07 &   \textbf{96.0$\pm$3.20} &          95.33$\pm$1.60 &           92.00$\pm$2.61 &          94.67$\pm$3.33 \\
%         &     $ 20\% $ &          90.67$\pm$5.23 &            92.00$\pm$1.6 & 88.67$\pm$4.43 &          89.33$\pm$5.62 & \textbf{94.00$\pm$2.44} &          89.33$\pm$6.98 &           90.67$\pm$3.20 \\
%        iris &     $ 30\% $ &          94.00$\pm$5.23 &          93.33$\pm$4.13 & 88.00$\pm$6.06 &           92.0$\pm$3.33 &         90.00$\pm$10.12 &          92.67$\pm$5.23 & \textbf{95.33$\pm$2.61} \\
%         &     $ 40\% $ & \textbf{90.67$\pm$4.33} &           84.00$\pm$7.28 &   78.00$\pm$5.7 &          88.67$\pm$3.33 &          82.00$\pm$9.82 &          84.67$\pm$5.31 &          86.67$\pm$9.91 \\
%         &     $ 50\% $ & \textbf{86.67$\pm$4.62} &           68.0$\pm$7.04 &  80.00$\pm$9.24 &          78.67$\pm$5.31 &          86.00$\pm$5.62 &           79.33$\pm$4.80 &           80.0$\pm$5.47 \\
% \midrule
%  &     $ 10\% $ &          93.49$\pm$3.35 &          92.09$\pm$3.09 & 92.09$\pm$2.32 & \textbf{93.49$\pm$3.02} &         88.84$\pm$4.87 & \textbf{93.49$\pm$3.02} &          92.09$\pm$3.09 \\
%  &     $ 20\% $ &           90.70$\pm$4.08 & \textbf{91.63$\pm$2.32} & 86.05$\pm$2.04 &          88.37$\pm$4.32 &         84.65$\pm$3.41 &          87.44$\pm$5.32 &          91.16$\pm$3.65 \\
% Thyroid &     $ 30\% $ &  \textbf{90.70$\pm$3.22} &          89.77$\pm$3.97 & 84.19$\pm$3.35 &          85.12$\pm$4.47 &         79.53$\pm$6.18 &          86.51$\pm$6.35 &           89.77$\pm$3.7 \\
%  &     $ 40\% $ & \textbf{88.84$\pm$3.35} &          86.51$\pm$2.66 &  82.79$\pm$3.70 &          83.26$\pm$2.23 &         80.47$\pm$5.32 &          87.91$\pm$4.42 &          88.84$\pm$5.08 \\
%  &     $ 50\% $ &          83.72$\pm$5.77 &          85.12$\pm$2.73 & 79.53$\pm$0.91 &          78.14$\pm$4.91 &          72.09$\pm$5.2 &          69.77$\pm$3.81 & \textbf{86.51$\pm$4.87} \\
% \midrule
%        &     $ 10\% $ &          56.67$\pm$2.15 &  \textbf{57.34$\pm$2.00} &  55.66$\pm$1.2 &          55.19$\pm$1.85 &         55.32$\pm$1.87 &           56.0$\pm$2.14 &          56.81$\pm$2.07 \\
%        &     $ 20\% $ & \textbf{54.05$\pm$2.51} &          53.71$\pm$3.41 & 52.23$\pm$2.55 &          50.14$\pm$1.49 &         49.46$\pm$1.29 &          48.86$\pm$1.02 &          52.83$\pm$1.63 \\
%       yeast &     $ 30\% $ &          50.61$\pm$2.12 & \textbf{50.81$\pm$3.33} & 48.78$\pm$4.08 &          46.56$\pm$2.51 &         46.02$\pm$2.91 &          45.82$\pm$2.82 &          50.27$\pm$1.49 \\
%        &     $ 40\% $ & \textbf{47.71$\pm$4.41} &          46.23$\pm$3.44 & 41.51$\pm$3.22 &          42.18$\pm$3.16 &         39.42$\pm$3.38 &          45.56$\pm$4.03 &          46.97$\pm$3.47 \\
%        &     $ 50\% $ & \textbf{42.25$\pm$1.99} &          41.58$\pm$1.87 & 38.42$\pm$3.18 &          37.53$\pm$1.79 &          36.32$\pm$2.10&          34.91$\pm$2.55 &          41.38$\pm$2.04 \\
% \bottomrule

% \end{tabular}
% \end{sc}
% \end{small}
% \end{center}
% \label{acc-on-randomly-missing-dataset}
% \vskip -0.1in
% \end{table*}
%-----------------------------------------------------------------------------------
% \begin{table}[ht]
%     \caption{Accuracy results on imputed data}
%     \setlength{\tabcolsep}{1.5 pt}
%     \label{tab-acc-randomly-missing}
%     \vskip 0.15in
%     \begin{center}
%     \begin{small}
%     \begin{sc}
% \begin{tabular}{lcccccccr}
% \toprule
%     dataset & missing rate &                   DIMV &               imputePCA &      KNNI &                    mice &             ALS &                    GAIN &                    GINN \\
% \midrule
%         &     $ 10\% $ &          95.33$\pm$2.61 &           92.67$\pm$3.2 & 93.33$\pm$2.07 &   \textbf{96.0$\pm$3.2} &          95.33$\pm$1.6 &           92.0$\pm$2.61 &          94.67$\pm$3.33 \\
%         &     $ 20\% $ &          92.67$\pm$2.44 &            92.0$\pm$1.6 & 88.67$\pm$4.43 &          89.33$\pm$5.62 & \textbf{94.0$\pm$2.44} &          89.33$\pm$6.98 &           90.67$\pm$3.2 \\
%        iris &     $ 30\% $ &           93.33$\pm$6.2 &          93.33$\pm$4.13 &  88.0$\pm$6.06 &           92.0$\pm$3.33 &         90.0$\pm$10.12 &          92.67$\pm$5.23 & \textbf{95.33$\pm$2.61} \\
%         &     $ 40\% $ & \textbf{91.33$\pm$3.33} &           84.0$\pm$7.28 &   78.0$\pm$5.7 &          88.67$\pm$3.33 &          82.0$\pm$9.82 &          84.67$\pm$5.31 &          86.67$\pm$9.91 \\
%         &     $ 50\% $ &           84.0$\pm$5.23 &           68.0$\pm$7.04 &  80.0$\pm$9.24 &          78.67$\pm$5.31 & \textbf{86.0$\pm$5.62} &           79.33$\pm$4.8 &           80.0$\pm$5.47 \\
% \midrule
%  &     $ 10\% $ &          \textbf{93.49$\pm$2.66} &          92.09$\pm$3.09 & 92.09$\pm$2.32 & \textbf{93.49$\pm$3.02} &         88.84$\pm$4.87 & \textbf{93.49$\pm$3.02} &          92.09$\pm$3.09 \\
%  &     $ 20\% $ &          90.23$\pm$1.71 & \textbf{91.63$\pm$2.32} & 86.05$\pm$2.04 &          88.37$\pm$4.32 &         84.65$\pm$3.41 &          87.44$\pm$5.32 &          91.16$\pm$3.65 \\
% thyroid &     $ 30\% $ &           89.3$\pm$4.23 & \textbf{89.77$\pm$3.97} & 84.19$\pm$3.35 &          85.12$\pm$4.47 &         79.53$\pm$6.18 &          86.51$\pm$6.35 &           89.77$\pm$3.7 \\
%  &     $ 40\% $ & \textbf{88.84$\pm$3.35} &          86.51$\pm$2.66 &  82.79$\pm$3.7 &          83.26$\pm$2.23 &         80.47$\pm$5.32 &          87.91$\pm$4.42 &          88.84$\pm$5.08 \\
%  &     $ 50\% $ &          84.65$\pm$4.23 &          85.12$\pm$2.73 & 79.53$\pm$0.91 &          78.14$\pm$4.91 &          72.09$\pm$5.2 &          69.77$\pm$3.81 & \textbf{86.51$\pm$4.87} \\
% \midrule
%        &     $ 10\% $ &           56.6$\pm$2.16 &  \textbf{57.34$\pm$2.0} &  55.66$\pm$1.2 &          55.19$\pm$1.85 &         55.32$\pm$1.87 &           56.0$\pm$2.14 &          56.81$\pm$2.07 \\
%        &     $ 20\% $ &          53.44$\pm$2.74 & \textbf{53.71$\pm$3.41} & 52.23$\pm$2.55 &          50.14$\pm$1.49 &         49.46$\pm$1.29 &          48.86$\pm$1.02 &          52.83$\pm$1.63 \\
%       yeast &     $ 30\% $ &  \textbf{51.01$\pm$2.0} &          50.81$\pm$3.33 & 48.78$\pm$4.08 &          46.56$\pm$2.51 &         46.02$\pm$2.91 &          45.82$\pm$2.82 &          50.27$\pm$1.49 \\
      
%        &     $ 40\% $ & \textbf{47.24$\pm$4.64} &          46.23$\pm$3.44 & 41.51$\pm$3.22 &          42.18$\pm$3.16 &         39.42$\pm$3.38 &          45.56$\pm$4.03 &          46.97$\pm$3.47 \\
%        &     $ 50\% $ & \textbf{41.85$\pm$2.03} &          41.58$\pm$1.87 & 38.42$\pm$3.18 &          37.53$\pm$1.79 &          36.32$\pm$2.1 &          34.91$\pm$2.55 &          41.38$\pm$2.04 \\
% \bottomrule

% \end{tabular}
% \end{sc}
% \end{small}
% \end{center}
% \label{acc-on-randomly-missing-dataset}
% \vskip -0.1in
% \end{table}


%-----------------------------------------------------------------------------------
\begin{table*}[ht]
    \caption{Accuracy results of imputed data}
    \setlength{\tabcolsep}{1.5 pt}
    \label{tab-acc-tabular1}
    \vskip 0.15in
    \begin{center}
    \begin{small}
    \begin{sc}
\begin{tabular}{lccccccccr}
\toprule
    dataset & missing rate &                    DIMV &            imputePCA &       KNNI &            mice &      ALS &            GAIN &                   GINN \\
\midrule
&     $ 10\% $ &          95.33$\pm$2.61 &  92.67$\pm$3.2 & 93.33$\pm$2.07 &   \textbf{96.0$\pm$3.2} &          95.33$\pm$1.6 &           92.0$\pm$2.61 &          94.67$\pm$3.33 \\
&     $ 20\% $ &          92.67$\pm$2.44 &   92.0$\pm$1.6 & 88.67$\pm$4.43 &          89.33$\pm$5.62 & \textbf{94.0$\pm$2.44} &          89.33$\pm$6.98 &           90.67$\pm$3.2 \\
iris &     $ 30\% $ &           93.33$\pm$6.2 & 93.33$\pm$4.13 &  88.0$\pm$6.06 &           92.0$\pm$3.33 &         90.0$\pm$10.12 &          92.67$\pm$5.23 & \textbf{95.33$\pm$2.61} \\
&     $ 40\% $ & \textbf{91.33$\pm$3.33} &  84.0$\pm$7.28 &   78.0$\pm$5.7 &          88.67$\pm$3.33 &          82.0$\pm$9.82 &          84.67$\pm$5.31 &          86.67$\pm$9.91 \\
&     $ 50\% $ &           84.0$\pm$5.23 &  68.0$\pm$7.04 &  80.0$\pm$9.24 &          78.67$\pm$5.31 &          86.0$\pm$5.62 &           79.33$\pm$4.8 &           80.0$\pm$5.47 \\
\midrule
&     $ 10\% $ &          93.49$\pm$2.66 & 92.09$\pm$3.09 & 92.09$\pm$2.32 & \textbf{93.49$\pm$3.02} &         88.84$\pm$4.87 & \textbf{93.49$\pm$3.02} &          92.09$\pm$3.09 \\
&     $ 20\% $ &          90.23$\pm$1.71 & 91.63$\pm$2.32 & 86.05$\pm$2.04 &          88.37$\pm$4.32 &         84.65$\pm$3.41 &          87.44$\pm$5.32 &          91.16$\pm$3.65 \\
thyroid &     $ 30\% $ &           89.3$\pm$4.23 & 89.77$\pm$3.97 & 84.19$\pm$3.35 &          85.12$\pm$4.47 &         79.53$\pm$6.18 &          86.51$\pm$6.35 &           89.77$\pm$3.7 \\
&     $ 40\% $ &          88.84$\pm$3.35 & 86.51$\pm$2.66 &  82.79$\pm$3.7 &          83.26$\pm$2.23 &         80.47$\pm$5.32 &          87.91$\pm$4.42 &          88.84$\pm$5.08 \\
&     $ 50\% $ &          84.65$\pm$4.23 & 85.12$\pm$2.73 & 79.53$\pm$0.91 &          78.14$\pm$4.91 &          72.09$\pm$5.2 &          69.77$\pm$3.81 &          86.51$\pm$4.87 \\
       
\midrule
&     $ 10\% $ &           56.6$\pm$2.16 &  57.34$\pm$2.0 &  55.66$\pm$1.2 &          55.19$\pm$1.85 &         55.32$\pm$1.87 &           56.0$\pm$2.14 &          56.81$\pm$2.07 \\
&     $ 20\% $ &          53.44$\pm$2.74 & 53.71$\pm$3.41 & 52.23$\pm$2.55 &          50.14$\pm$1.49 &         49.46$\pm$1.29 &          48.86$\pm$1.02 &          52.83$\pm$1.63 \\
yeast &     $ 30\% $ &  \textbf{51.01$\pm$2.0} & 50.81$\pm$3.33 & 48.78$\pm$4.08 &          46.56$\pm$2.51 &         46.02$\pm$2.91 &          45.82$\pm$2.82 &          50.27$\pm$1.49 \\
  &     $ 40\% $ & \textbf{47.24$\pm$4.64} & 46.23$\pm$3.44 & 41.51$\pm$3.22 &          42.18$\pm$3.16 &         39.42$\pm$3.38 &          45.56$\pm$4.03 &          46.97$\pm$3.47 \\
  &     $ 50\% $ & \textbf{41.85$\pm$2.03} & 41.58$\pm$1.87 & 38.42$\pm$3.18 &          37.53$\pm$1.79 &          36.32$\pm$2.1 &          34.91$\pm$2.55 &          41.38$\pm$2.04 \\
\bottomrule
\end{tabular}
\end{sc}
\end{small}
\end{center}
\label{tab-rmse-on-randomly-missing-dataset}
\vskip -0.1in
\end{table*} 

==> formated_algos/table_5.2.2.2_extra.tex <==
\begin{table}[ht]
    \caption{Accuracy results on imputed data}
    \setlength{\tabcolsep}{1.5 pt}
    \label{tab-acc-randomly-missing}
    \vskip 0.15in
    \begin{center}
    \begin{small}
    \begin{sc}
\begin{tabular}{lcccccccr}
\toprule
    dataset & missing rate &              missForest &             EM &                 MeanImp \\
\midrule
        &     $ 10\% $ &           94.67$\pm$1.6 & 95.33$\pm$2.61 &          92.67$\pm$3.81 \\
        &     $ 20\% $ &          93.33$\pm$2.92 &  90.67$\pm$3.2 &           92.67$\pm$3.2 \\
       iris &     $ 30\% $ & \textbf{95.33$\pm$3.92} & 93.33$\pm$4.62 &          93.33$\pm$2.92 \\
        &     $ 40\% $ &          90.67$\pm$3.81 &  90.0$\pm$2.92 &          87.33$\pm$5.62 \\
        &     $ 50\% $ & \textbf{87.33$\pm$3.81} & 82.67$\pm$6.66 &           84.0$\pm$6.33 \\
\midrule        
        
        
 &     $ 10\% $ &           93.02$\pm$2.5 & 93.02$\pm$1.44 &          91.63$\pm$2.73 \\
 &     $ 20\% $ & \textbf{92.09$\pm$2.73} & 90.23$\pm$3.65 &            90.7$\pm$2.5 \\
thyroid &     $ 30\% $ &  \textbf{92.09$\pm$3.7} & 86.51$\pm$2.66 &          88.37$\pm$3.22 \\
 &     $ 40\% $ &           89.3$\pm$4.23 & 84.19$\pm$3.02 &  \textbf{90.7$\pm$4.08} \\
 &     $ 50\% $ &          86.51$\pm$3.92 & 72.09$\pm$2.88 & \textbf{86.98$\pm$4.23} \\
 
 \midrule
 
       &     $ 10\% $ & \textbf{57.41$\pm$1.56} & 55.52$\pm$2.47 &           56.8$\pm$1.96 \\
       &     $ 20\% $ & \textbf{54.11$\pm$2.77} & 50.34$\pm$1.52 &          51.96$\pm$2.76 \\
      yeast &     $ 30\% $ &           49.8$\pm$3.97 & 48.11$\pm$1.49 &          50.74$\pm$1.87 \\
       &     $ 40\% $ &          45.42$\pm$2.93 & 41.11$\pm$3.56 &           46.7$\pm$3.67 \\
       &     $ 50\% $ &          41.04$\pm$1.97 & 39.01$\pm$2.61 &          41.58$\pm$1.46 \\
\bottomrule
\end{tabular}
\end{sc}
\end{small}
\end{center}
\label{acc-on-randomly-missing-dataset}
\vskip -0.1in
\end{table}


==> formated_algos/table_5.2.2.2_extra_v2.tex <==
\begin{table*}[ht]
    \caption{Accuracy results on imputed data}
    \setlength{\tabcolsep}{1.5 pt}
    \label{tab-acc-randomly-missing}
    \vskip 0.15in
    \begin{center}
    \begin{small}
    \begin{sc}
\begin{tabular}{lcccr}
\toprule
    dataset & missing rate &               missForest &              EM &         MeanImp \\
    \midrule
     &     $ 10\% $ &           94.67$\pm$1.6 & 95.33$\pm$2.61 &         93.33$\pm$5.47 \\
     &     $ 20\% $ &          93.33$\pm$2.92                &  90.67$\pm$3.2 &          92.67$\pm$3.2 \\
    iris &     $ 30\% $ & \textbf{95.33$\pm$3.92} & 93.33$\pm$4.62 &          94.0$\pm$2.44 \\
     &     $ 40\% $ &          90.67$\pm$3.81 &  90.0$\pm$2.92 &          90.0$\pm$2.07 \\
      &     $ 50\% $ & \textbf{87.33$\pm$3.81} & 82.67$\pm$6.66 &          82.0$\pm$6.06 \\

    \midrule
 &     $ 10\% $ &           93.02$\pm$2.5 & 93.02$\pm$1.44 &         92.09$\pm$3.09 \\
 &     $ 20\% $ & \textbf{92.09$\pm$2.73} & 90.23$\pm$3.65 &          90.7$\pm$1.44 \\
thyroid &     $ 30\% $ &  \textbf{92.09$\pm$3.7} & 86.51$\pm$2.66 &         86.98$\pm$3.97 \\
 &     $ 40\% $ &           89.3$\pm$4.23 & 84.19$\pm$3.02 &         88.84$\pm$5.84 \\
 &     $ 50\% $ & \textbf{86.51$\pm$3.92} & 72.09$\pm$2.88 &         83.72$\pm$4.56 \\
   \midrule
    &     $ 10\% $ & \textbf{57.41$\pm$1.56} & 55.52$\pm$2.47 &         56.67$\pm$2.15 \\
    &     $ 20\% $ & \textbf{54.11$\pm$2.77} & 50.34$\pm$1.52 &         52.03$\pm$2.87 \\
   yeast &     $ 30\% $ &           49.8$\pm$3.97 & 48.11$\pm$1.49 &          50.2$\pm$2.32 \\
    &     $ 40\% $ &          45.42$\pm$2.93 & 41.11$\pm$3.56 &         45.56$\pm$4.31 \\
    &     $ 50\% $ &          41.04$\pm$1.97 & 39.01$\pm$2.61 &          41.38$\pm$2.1 \\
\bottomrule
\end{tabular}
\end{sc}
\end{small}
\end{center}
%\label{tab-rmse-on-randomly-missing-dataset}
\vskip -0.1in
\end{table*}

==> formated_algos/table_5.2.2.2_v2.tex <==
\begin{table*}[ht]
    \caption{Accuracy results of imputed data}
    \setlength{\tabcolsep}{1.5 pt}
    \label{tab-acc-tabular1}
    \vskip 0.15in
    \begin{center}
    \begin{small}
    \begin{sc}
\begin{tabular}{lccccccccr}
\toprule
    dataset & missing rate &                    DIMV &            imputePCA &       KNNI &            mice &      ALS &            GAIN &                   GINN \\
    \midrule
     &     $ 10\% $ &          95.33$\pm$2.61 &  92.67$\pm$3.2 & 93.33$\pm$2.07 &   \textbf{96.0$\pm$3.2} &          95.33$\pm$1.6 &           92.0$\pm$2.61 &          94.67$\pm$3.33 \\
     &     $ 20\% $ &          92.67$\pm$2.44 &   92.0$\pm$1.6 & 88.67$\pm$4.43 &          89.33$\pm$5.62 & \textbf{94.0$\pm$2.44} &          89.33$\pm$6.98 &           90.67$\pm$3.2 \\
    iris &     $ 30\% $ &           93.33$\pm$6.2 & 93.33$\pm$4.13 &  88.0$\pm$6.06 &           92.0$\pm$3.33 &         90.0$\pm$10.12 &          92.67$\pm$5.23 & \textbf{95.33$\pm$2.61} \\
     &     $ 40\% $ & \textbf{91.33$\pm$3.33} &  84.0$\pm$7.28 &   78.0$\pm$5.7 &          88.67$\pm$3.33 &          82.0$\pm$9.82 &          84.67$\pm$5.31 &          86.67$\pm$9.91 \\
     &     $ 50\% $ &           84.0$\pm$5.23 &  68.0$\pm$7.04 &  80.0$\pm$9.24 &          78.67$\pm$5.31 &          86.0$\pm$5.62 &           79.33$\pm$4.8 &           80.0$\pm$5.47 \\

    \midrule
        &     $ 10\% $ &          93.49$\pm$2.66 & 92.09$\pm$3.09 & 92.09$\pm$2.32 & \textbf{93.49$\pm$3.02} &         88.84$\pm$4.87 & \textbf{93.49$\pm$3.02} &          92.09$\pm$3.09 \\
 &     $ 20\% $ &          90.23$\pm$1.71 & 91.63$\pm$2.32 & 86.05$\pm$2.04  &          88.37$\pm$4.32 &         84.65$\pm$3.41 &          87.44$\pm$5.32 &          91.16$\pm$3.65 \\
 
thyroid &     $ 30\% $ &           89.3$\pm$4.23 & 89.77$\pm$3.97 & 84.19$\pm$3.35 &          85.12$\pm$4.47 &         79.53$\pm$6.18 &          86.51$\pm$6.35 &           89.77$\pm$3.7 \\
&     $ 40\% $ &          88.84$\pm$3.35 & 86.51$\pm$2.66 &  82.79$\pm$3.7 &          83.26$\pm$2.23 &         80.47$\pm$5.32 &          87.91$\pm$4.42 &          88.84$\pm$5.08 \\
&     $ 50\% $ &          84.65$\pm$4.23 & 85.12$\pm$2.73 & 79.53$\pm$0.91 &          78.14$\pm$4.91 &          72.09$\pm$5.2 &          69.77$\pm$3.81 &          86.51$\pm$4.87 \\
\midrule 
    &     $ 10\% $ &           56.6$\pm$2.16 &  57.34$\pm$2.0 &  55.66$\pm$1.2 &          55.19$\pm$1.85 &         55.32$\pm$1.87 &           56.0$\pm$2.14 &          56.81$\pm$2.07 \\
    &     $ 20\% $ &          53.44$\pm$2.74 & 53.71$\pm$3.41 & 52.23$\pm$2.55 &          50.14$\pm$1.49 &         49.46$\pm$1.29 &          48.86$\pm$1.02 &          52.83$\pm$1.63 \\
   yeast &     $ 30\% $ &  \textbf{51.01$\pm$2.0} & 50.81$\pm$3.33 & 48.78$\pm$4.08 &          46.56$\pm$2.51 &         46.02$\pm$2.91 &          45.82$\pm$2.82 &          50.27$\pm$1.49 \\
    &     $ 40\% $ & \textbf{47.24$\pm$4.64} & 46.23$\pm$3.44 & 41.51$\pm$3.22 &          42.18$\pm$3.16 &         39.42$\pm$3.38 &          45.56$\pm$4.03 &          46.97$\pm$3.47 \\
    &     $ 50\% $ &          41.85$\pm$2.03 & 41.58$\pm$1.87 & 38.42$\pm$3.18 &          37.53$\pm$1.79 &          36.32$\pm$2.1 &          34.91$\pm$2.55 &          41.38$\pm$2.04 \\
\bottomrule
\end{tabular}
\end{sc}
\end{small}
\end{center}
\label{tab-rmse-on-randomly-missing-dataset}
\vskip -0.1in
\end{table*} 

==> formated_algos/table_5.2.3.1.tex <==

 


% \begin{table*}[ht]
%     \caption{RMSE for GAIN, ALS and DIMV on MNIST under different missing rates.}
%     \setlength{\tabcolsep}{1 pt}
%     \label{sample-table}
%     \vskip 0.15in
%     \begin{center}
%     \begin{small}
%     \begin{sc}
%     \begin{tabular}{lccccr}
%         \toprule
%         missing rates &  GAIN & ALS &  DIMV  \\
%         \midrule
% 40\%  & 126.5  $\pm$  5.6 \; &  104.9  $\pm$  0.2 \; &  \textbf{97.7  $\pm$  1.1}\\
% 50\%  & 184.4  $\pm$  1.7 \; & 159.6  $\pm$  17.8 \; & \textbf{140.7  $\pm$  1.1} \\
% 60\% & 201.3  $\pm$  2.9 \; &  154.9  $\pm$  0.5 \;& \textbf{149.6  $\pm$  1.0} \\ 
%         \bottomrule

%     \end{tabular}
%     \end{sc}
%     \end{small}
%     \end{center}
%     \vskip -0.1in
% \end{table*} 


\begin{table}[ht]
    \caption{RMSE under different missing rates. The methods that cannot deliver results in 5 hours are removed from the table. }
    \label{tab-rmse-mnist}
    \setlength{\tabcolsep}{1.3 pt}
    \vskip 0.15in
    \begin{center}
    \begin{small}
    \begin{sc}
    \begin{tabular}{lccccr}
        \toprule
        dataset & missing rates &  GAIN & kNNI & ALS &  DIMV  \\
        \midrule
           & 40\% & 110.57       &  53.64  & 55.93 & \textbf{39.36}  \\
          Mnist & 50\% & 122.88  &  72.50  & 70.55 & \textbf{54.20} \\
           & 60\% & 110.89       &  80.49  & 74.73 & \textbf{60.99} \\ 
        \midrule
                        & 40\% & 124.54  & 80.07 & 41.77 & \textbf{25.32}  \\
          Fashion-MNIST & 50\% & 130.07  & 86.64 & 61.90 & \textbf{39.03}  \\
                        & 60\% & 133.70  & 90.92 & 63.79 & \textbf{42.13} \\ 
        \bottomrule
    \end{tabular}
    \end{sc}
    \end{small}
    \end{center}
    \vskip -0.1in
\end{table}  

==> formated_algos/table_5.2.3.2.tex <==

% \begin{table*}[ht]
%     \caption{Classification accuracies for GAIN, ALS and DIMV on MNIST with different missing rates.} 
%     \setlength{\tabcolsep}{1.2 pt}
%     \label{sample-table}
%     \vskip 0.15in
%     \begin{center}
%     \begin{small}
%     \begin{sc}
%     \begin{tabular}{lccccr}
%         \toprule
%         missing rates  &  GAIN & ALS &  DIMV  \\
%         \midrule
% 40\% & 97.31  $\pm$  0.15 \;& 97.46  $\pm$  0.07 \;& \textbf{97.59  $\pm$  0.02} \\
% 50\%  &  95.47  $\pm$  0.4 \; & 96.59  $\pm$  0.15 \; & \textbf{97.24  $\pm$  0.09} \\
% 60\%  & 89.39  $\pm$  0.76 \; & 94.22  $\pm$  0.13 \;& \textbf{95.78  $\pm$  0.11} \\ 
%         \bottomrule
        
%         \bottomrule
%     \end{tabular}
%     \end{sc}
%     \end{small}
%     \end{center}
%     \vskip -0.1in
% \end{table*}   







\begin{table}[ht]
    \caption{Classification accuracies under various missing rates. The methods that cannot deliver results in 5 hours are removed from the table.} 
    \setlength{\tabcolsep}{1.6pt}
    \label{tab-acc-mnist}
    \vskip 0.15in
    \begin{center}
    \begin{small}
    \begin{sc}
    \begin{tabular}{lccccr}
        \toprule
       dataset &  missing rates  &  GAIN & KNNI & ALS &  DIMV  \\
        \midrule
                  & 40\% & 97.13 & 97.65 & 97.51   & \textbf{97.79} \\
            Mnist & 50\% & 95.54 & \textbf{97.23}  & 96.36 & 97.11 \\
                  & 60\% & 86.35 & 95.08 & 94.33   & \textbf{95.78} \\
            \midrule
                        & 40\% & 88.93 & \textbf{89.45} & 89.28 & 88.99  \\
          Fashion-MNIST & 50\% & 87.42 & 88.78 & 88.82  & \textbf{88.92}  \\
                        & 60\% & 85.97 & 88.94 & 88.74  & \textbf{88.57} \\ 
        \bottomrule
    \end{tabular}
    \end{sc}
    \end{small}
    \end{center}
    \vskip -0.1in
\end{table}   


==> formated_algos/table_rmse_rand_nips_1.tex <==
\begin{table}[ht]
    \caption{RMSE values were evaluated for various missing rates in tabular datasets. The best, second best, and third best results were highlighted with \textbf{bold}, \textit{italic}, and \underline{underline} respectively.}\label{table:rand-rmse}
    \setlength{\tabcolsep}{1.3 pt}
    \vskip 0.15in
    \begin{center}
    \begin{small}
    \begin{sc}
\begin{tabular}{lllllll}
\toprule
      dataset & missing\_rate &                                           dimv &                                             em &               gain &                                      imputepca &                                           mean \\
\midrule
iris & 0.1 &  $\underline{ 0.336 } \pm \underline{ 0.068 }$ &                              $0.464 \pm 0.075$ &  $0.803 \pm 0.205$ &                              $0.341 \pm 0.057$ &                              $1.106 \pm 0.111$ \\
      & 0.2 &                              $0.408 \pm 0.037$ &                              $0.542 \pm 0.059$ &  $0.878 \pm 0.143$ &        $\textit{ 0.399 } \pm \textit{ 0.048 }$ &                              $1.084 \pm 0.052$ \\
      & 0.3 &                              $0.476 \pm 0.059$ &                              $0.612 \pm 0.101$ &  $0.796 \pm 0.154$ &  $\underline{ 0.456 } \pm \underline{ 0.020 }$ &                              $1.074 \pm 0.059$ \\
      & 0.4 &                              $0.581 \pm 0.068$ &                              $0.697 \pm 0.079$ &  $0.928 \pm 0.128$ &        $\textit{ 0.534 } \pm \textit{ 0.048 }$ &                              $1.075 \pm 0.038$ \\
      & 0.5 &                              $0.694 \pm 0.066$ &                              $0.771 \pm 0.088$ &  $1.072 \pm 0.119$ &        $\mathbf{ 0.595 } \pm \mathbf{ 0.076 }$ &                              $1.055 \pm 0.049$ \\
      & 0.6 &                              $0.763 \pm 0.064$ &                              $0.801 \pm 0.101$ &  $1.051 \pm 0.124$ &        $\mathbf{ 0.689 } \pm \mathbf{ 0.075 }$ &                              $1.083 \pm 0.044$ \\
      & 0.7 &        $\textit{ 0.877 } \pm \textit{ 0.041 }$ &                              $0.954 \pm 0.115$ &  $1.097 \pm 0.089$ &        $\mathbf{ 0.795 } \pm \mathbf{ 0.072 }$ &                              $1.098 \pm 0.060$ \\
      & 0.8 &                              $0.999 \pm 0.050$ &  $\underline{ 0.978 } \pm \underline{ 0.119 }$ &  $1.087 \pm 0.069$ &        $\textit{ 0.915 } \pm \textit{ 0.110 }$ &                              $1.093 \pm 0.063$ \\
      \midrule
thyroid & 0.1 &                              $6.721 \pm 0.928$ &                              $8.854 \pm 1.009$ &  $8.988 \pm 1.414$ &        $\mathbf{ 5.465 } \pm \mathbf{ 0.650 }$ &                              $7.894 \pm 0.780$ \\
      & 0.2 &  $\underline{ 6.473 } \pm \underline{ 0.703 }$ &                              $8.827 \pm 1.324$ &  $8.264 \pm 1.247$ &        $\mathbf{ 5.654 } \pm \mathbf{ 0.772 }$ &                              $7.646 \pm 0.550$ \\
      & 0.3 &  $\underline{ 6.661 } \pm \underline{ 0.618 }$ &                              $9.146 \pm 0.685$ &  $8.405 \pm 2.339$ &        $\mathbf{ 6.397 } \pm \mathbf{ 0.884 }$ &                              $7.553 \pm 0.683$ \\
      & 0.4 &        $\textit{ 7.070 } \pm \textit{ 0.686 }$ &                              $9.276 \pm 0.913$ &  $9.028 \pm 1.910$ &        $\mathbf{ 6.769 } \pm \mathbf{ 0.648 }$ &                              $8.068 \pm 0.607$ \\
      & 0.5 &  $\underline{ 7.242 } \pm \underline{ 0.593 }$ &                              $9.313 \pm 0.668$ &  $9.076 \pm 0.846$ &        $\mathbf{ 6.537 } \pm \mathbf{ 0.507 }$ &                              $7.906 \pm 0.582$ \\
      & 0.6 &        $\mathbf{ 7.164 } \pm \mathbf{ 0.213 }$ &                              $9.575 \pm 0.637$ &  $8.486 \pm 0.494$ &                              $7.711 \pm 0.710$ &                              $7.772 \pm 0.348$ \\
      & 0.7 &        $\mathbf{ 7.361 } \pm \mathbf{ 0.271 }$ &                              $9.752 \pm 0.858$ &  $9.048 \pm 1.144$ &                              $9.629 \pm 2.129$ &  $\underline{ 7.809 } \pm \underline{ 0.300 }$ \\
      & 0.8 &        $\textit{ 8.006 } \pm \textit{ 0.417 }$ &                              $9.509 \pm 0.925$ &  $8.801 \pm 0.662$ &                              $9.606 \pm 1.133$ &  $\underline{ 8.050 } \pm \underline{ 0.425 }$ \\
      \midrule
seeds & 0.1 &        $\textit{ 0.470 } \pm \textit{ 0.073 }$ &                              $0.598 \pm 0.082$ &  $0.757 \pm 0.126$ &                              $0.625 \pm 0.058$ &                              $1.306 \pm 0.107$ \\
      & 0.2 &  $\underline{ 0.547 } \pm \underline{ 0.069 }$ &                              $0.693 \pm 0.099$ &  $0.821 \pm 0.114$ &                              $0.631 \pm 0.087$ &                              $1.378 \pm 0.079$ \\
      & 0.3 &        $\textit{ 0.598 } \pm \textit{ 0.058 }$ &                              $0.787 \pm 0.072$ &  $0.829 \pm 0.090$ &                              $0.727 \pm 0.056$ &                              $1.386 \pm 0.049$ \\
      & 0.4 &        $\textit{ 0.661 } \pm \textit{ 0.108 }$ &                              $0.781 \pm 0.080$ &  $0.875 \pm 0.086$ &  $\underline{ 0.704 } \pm \underline{ 0.068 }$ &                              $1.399 \pm 0.029$ \\
      & 0.5 &  $\underline{ 0.779 } \pm \underline{ 0.134 }$ &                              $0.885 \pm 0.102$ &  $1.027 \pm 0.204$ &        $\textit{ 0.776 } \pm \textit{ 0.045 }$ &                              $1.364 \pm 0.058$ \\
      & 0.6 &  $\underline{ 0.870 } \pm \underline{ 0.121 }$ &                              $0.971 \pm 0.066$ &  $1.150 \pm 0.165$ &        $\textit{ 0.861 } \pm \textit{ 0.075 }$ &                              $1.356 \pm 0.036$ \\
      & 0.7 &  $\underline{ 1.034 } \pm \underline{ 0.114 }$ &                              $1.105 \pm 0.139$ &  $1.304 \pm 0.106$ &        $\textit{ 0.967 } \pm \textit{ 0.102 }$ &                              $1.370 \pm 0.033$ \\
      & 0.8 &        $\textit{ 1.181 } \pm \textit{ 0.081 }$ &  $\underline{ 1.184 } \pm \underline{ 0.125 }$ &  $1.391 \pm 0.059$ &                              $1.199 \pm 0.130$ &                              $1.381 \pm 0.024$ \\
      \midrule
yeast & 0.1 &        $\textit{ 0.093 } \pm \textit{ 0.004 }$ &                              $0.132 \pm 0.003$ &  $0.206 \pm 0.003$ &                              $0.096 \pm 0.003$ &                              $0.102 \pm 0.004$ \\
      & 0.2 &        $\textit{ 0.095 } \pm \textit{ 0.004 }$ &                              $0.133 \pm 0.002$ &  $0.205 \pm 0.004$ &  $\underline{ 0.095 } \pm \underline{ 0.004 }$ &                              $0.102 \pm 0.003$ \\
      & 0.3 &        $\mathbf{ 0.097 } \pm \mathbf{ 0.002 }$ &                              $0.135 \pm 0.002$ &  $0.207 \pm 0.004$ &        $\textit{ 0.098 } \pm \textit{ 0.002 }$ &                              $0.103 \pm 0.002$ \\
      & 0.4 &        $\mathbf{ 0.097 } \pm \mathbf{ 0.002 }$ &                              $0.136 \pm 0.001$ &  $0.207 \pm 0.003$ &        $\textit{ 0.101 } \pm \textit{ 0.002 }$ &  $\underline{ 0.103 } \pm \underline{ 0.002 }$ \\
      & 0.5 &        $\mathbf{ 0.098 } \pm \mathbf{ 0.002 }$ &                              $0.138 \pm 0.002$ &  $0.206 \pm 0.002$ &  $\underline{ 0.105 } \pm \underline{ 0.002 }$ &        $\textit{ 0.102 } \pm \textit{ 0.001 }$ \\
      & 0.6 &        $\mathbf{ 0.099 } \pm \mathbf{ 0.001 }$ &                              $0.139 \pm 0.001$ &  $0.207 \pm 0.005$ &                              $0.113 \pm 0.004$ &        $\textit{ 0.102 } \pm \textit{ 0.001 }$ \\
      & 0.7 &        $\mathbf{ 0.100 } \pm \mathbf{ 0.001 }$ &                              $0.141 \pm 0.002$ &  $0.208 \pm 0.004$ &                              $0.123 \pm 0.004$ &        $\textit{ 0.102 } \pm \textit{ 0.001 }$ \\
      & 0.8 &        $\textit{ 0.102 } \pm \textit{ 0.001 }$ &                              $0.143 \pm 0.003$ &  $0.212 \pm 0.006$ &                              $0.146 \pm 0.023$ &        $\mathbf{ 0.102 } \pm \mathbf{ 0.001 }$ \\
\bottomrule
\end{tabular}
    \end{sc}
    \end{small}
    \end{center}
    \vskip -0.1in
\end{table}    

==> formated_algos/table_rmse_rand_nips_2.tex <==
\begin{table}[ht]
    \caption{RMSE values were evaluated for various missing rates in tabular datasets. The best, second best, and third best results were highlighted with \textbf{bold}, \textit{italic}, and \underline{underline} respectively.}\label{table:rand-rmse-2}
    \setlength{\tabcolsep}{1.3 pt}
    \vskip 0.15in
    \begin{center}
    \begin{small}
    \begin{sc}
\begin{tabular}{llllll}
\toprule
      dataset & missing\_rate &                                            knn &                                           mice &                                     missforest &          softimpute \\
\midrule
iris & 0.1 &                              $0.449 \pm 0.074$ &        $\mathbf{ 0.311 } \pm \mathbf{ 0.062 }$ &        $\textit{ 0.315 } \pm \textit{ 0.039 }$ &   $0.858 \pm 0.125$ \\
      & 0.2 &                              $0.536 \pm 0.086$ &  $\underline{ 0.402 } \pm \underline{ 0.042 }$ &        $\mathbf{ 0.360 } \pm \mathbf{ 0.081 }$ &   $0.895 \pm 0.049$ \\
      & 0.3 &                              $0.618 \pm 0.062$ &        $\textit{ 0.447 } \pm \textit{ 0.044 }$ &        $\mathbf{ 0.441 } \pm \mathbf{ 0.067 }$ &   $0.970 \pm 0.076$ \\
      & 0.4 &                              $0.683 \pm 0.073$ &        $\mathbf{ 0.531 } \pm \mathbf{ 0.069 }$ &  $\underline{ 0.575 } \pm \underline{ 0.131 }$ &   $0.998 \pm 0.066$ \\
      & 0.5 &                              $0.761 \pm 0.077$ &  $\underline{ 0.645 } \pm \underline{ 0.090 }$ &        $\textit{ 0.638 } \pm \textit{ 0.091 }$ &   $1.055 \pm 0.041$ \\
      & 0.6 &                              $0.822 \pm 0.055$ &        $\textit{ 0.748 } \pm \textit{ 0.090 }$ &  $\underline{ 0.760 } \pm \underline{ 0.093 }$ &   $1.069 \pm 0.068$ \\
      & 0.7 &                              $0.908 \pm 0.051$ &  $\underline{ 0.879 } \pm \underline{ 0.105 }$ &                              $0.882 \pm 0.122$ &   $1.127 \pm 0.048$ \\
      & 0.8 &                              $1.078 \pm 0.085$ &                              $1.012 \pm 0.094$ &        $\mathbf{ 0.913 } \pm \mathbf{ 0.280 }$ &   $1.171 \pm 0.080$ \\
    \midrule
thyroid & 0.1 &  $\underline{ 5.834 } \pm \underline{ 0.461 }$ &                              $6.727 \pm 0.929$ &        $\textit{ 5.805 } \pm \textit{ 0.902 }$ &   $8.326 \pm 0.796$ \\
      & 0.2 &                              $6.866 \pm 0.658$ &                              $6.704 \pm 0.855$ &        $\textit{ 6.398 } \pm \textit{ 0.522 }$ &   $8.225 \pm 0.778$ \\
      & 0.3 &                              $7.001 \pm 0.583$ &                              $7.214 \pm 0.986$ &        $\textit{ 6.509 } \pm \textit{ 0.936 }$ &   $8.446 \pm 0.758$ \\
      & 0.4 &                              $7.437 \pm 0.750$ &                              $8.523 \pm 1.404$ &  $\underline{ 7.133 } \pm \underline{ 0.549 }$ &   $9.118 \pm 0.558$ \\
      & 0.5 &                              $7.445 \pm 0.419$ &                              $8.919 \pm 1.636$ &        $\textit{ 7.105 } \pm \textit{ 0.765 }$ &   $9.391 \pm 0.648$ \\
      & 0.6 &        $\textit{ 7.218 } \pm \textit{ 0.483 }$ &                              $9.220 \pm 1.752$ &  $\underline{ 7.677 } \pm \underline{ 0.710 }$ &   $9.545 \pm 0.849$ \\
      & 0.7 &        $\textit{ 7.523 } \pm \textit{ 0.416 }$ &                              $7.822 \pm 0.419$ &                              $7.959 \pm 0.613$ &   $9.925 \pm 0.869$ \\
      & 0.8 &        $\mathbf{ 7.807 } \pm \mathbf{ 0.459 }$ &                              $8.522 \pm 0.757$ &                              $8.728 \pm 0.895$ &  $10.361 \pm 0.903$ \\
      \midrule
seeds & 0.1 &                              $0.527 \pm 0.072$ &        $\mathbf{ 0.451 } \pm \mathbf{ 0.080 }$ &  $\underline{ 0.474 } \pm \underline{ 0.051 }$ &   $0.631 \pm 0.072$ \\
      & 0.2 &                              $0.668 \pm 0.076$ &        $\textit{ 0.539 } \pm \textit{ 0.048 }$ &        $\mathbf{ 0.533 } \pm \mathbf{ 0.078 }$ &   $0.740 \pm 0.067$ \\
      & 0.3 &                              $0.813 \pm 0.073$ &  $\underline{ 0.599 } \pm \underline{ 0.057 }$ &        $\mathbf{ 0.593 } \pm \mathbf{ 0.055 }$ &   $0.925 \pm 0.058$ \\
      & 0.4 &                              $0.931 \pm 0.064$ &                              $0.715 \pm 0.077$ &        $\mathbf{ 0.624 } \pm \mathbf{ 0.062 }$ &   $1.058 \pm 0.059$ \\
      & 0.5 &                              $1.019 \pm 0.051$ &                              $0.793 \pm 0.064$ &        $\mathbf{ 0.720 } \pm \mathbf{ 0.049 }$ &   $1.151 \pm 0.092$ \\
      & 0.6 &                              $1.012 \pm 0.043$ &                              $0.886 \pm 0.070$ &        $\mathbf{ 0.791 } \pm \mathbf{ 0.050 }$ &   $1.312 \pm 0.069$ \\
      & 0.7 &                              $1.059 \pm 0.065$ &                              $1.130 \pm 0.114$ &        $\mathbf{ 0.898 } \pm \mathbf{ 0.075 }$ &   $1.396 \pm 0.085$ \\
      & 0.8 &                              $1.203 \pm 0.071$ &                              $1.294 \pm 0.122$ &        $\mathbf{ 1.071 } \pm \mathbf{ 0.102 }$ &   $1.567 \pm 0.067$ \\
      \midrule
yeast & 0.1 &                              $0.103 \pm 0.003$ &        $\mathbf{ 0.092 } \pm \mathbf{ 0.004 }$ &  $\underline{ 0.094 } \pm \underline{ 0.003 }$ &   $0.108 \pm 0.006$ \\
      & 0.2 &                              $0.109 \pm 0.004$ &        $\mathbf{ 0.095 } \pm \mathbf{ 0.004 }$ &                              $0.099 \pm 0.003$ &   $0.110 \pm 0.003$ \\
      & 0.3 &                              $0.112 \pm 0.003$ &  $\underline{ 0.099 } \pm \underline{ 0.003 }$ &                              $0.104 \pm 0.002$ &   $0.111 \pm 0.003$ \\
      & 0.4 &                              $0.112 \pm 0.002$ &                              $0.120 \pm 0.004$ &                              $0.107 \pm 0.002$ &   $0.111 \pm 0.001$ \\
      & 0.5 &                              $0.111 \pm 0.001$ &                              $0.143 \pm 0.030$ &                              $0.113 \pm 0.003$ &   $0.114 \pm 0.002$ \\
      & 0.6 &  $\underline{ 0.112 } \pm \underline{ 0.001 }$ &                              $0.125 \pm 0.018$ &                              $0.117 \pm 0.005$ &   $0.119 \pm 0.002$ \\
      & 0.7 &  $\underline{ 0.110 } \pm \underline{ 0.001 }$ &                              $0.113 \pm 0.015$ &                              $0.120 \pm 0.006$ &   $0.123 \pm 0.002$ \\
      & 0.8 &  $\underline{ 0.109 } \pm \underline{ 0.001 }$ &                              $0.113 \pm 0.007$ &                              $0.128 \pm 0.007$ &   $0.130 \pm 0.002$ \\
\bottomrule
\end{tabular}
    \end{sc}
    \end{small}
    \end{center}
    \vskip -0.1in
\end{table}    
